GestureHYDRA: Semantic Co-speech Gesture Synthesis via Hybrid Modality Diffusion Transformer and Cascaded-Synchronized Retrieval-Augmented Generation

While increasing attention has been paid to co-speech gesture synthesis, most previous works neglect to investigate hand gestures with explicit and essential semantics. In this paper, we study co-speech gesture generation with an emphasis on specific hand gesture activation, which can deliver more instructional information than common body movements. To achieve this, we first build a high-quality dataset of 3D human body movements including a set of semantically explicit hand gestures that are commonly used by live streamers. Then we present a hybrid-modality gesture generation system GestureHYDRA built upon a hybrid-modality diffusion transformer architecture with novelly designed motion-style injective transformer layers, which enables advanced gesture modeling ability and versatile gesture operations. To guarantee these specific hand gestures can be activated, we introduce a cascaded retrieval-augmented generation strategy built upon a semantic gesture repository annotated for each subject and an adaptive audio-gesture synchronization mechanism, which substantially improves semantic gesture activation and production efficiency. Quantitative and qualitative experiments demonstrate that our proposed approach achieves superior performance over all the counterparts. The project page can be found at https://mumuwei.github.io/GestureHYDRA/.

==> sections/_preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% common preambles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%--------------------------------------------------
% colored text and comments
%--------------------------------------------------
\usepackage{bm}
\usepackage{bbm}

\usepackage{colortbl}
%--------------------------------------------------
% for vectors (should be surrounded by $)
%--------------------------------------------------
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{subcaption}
\usepackage{multirow}
%\usepackage{gensymb}
\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{mathtools}
\usepackage{mathrsfs}
\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
%\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\tildevect}[1]{\vect{\tilde{#1}}}
\newcommand{\hatvect}[1]{\vect{\hat{#1}}}
\newcommand{\overlinevect}[1]{\vect{\overline{#1}}}
\newcommand{\unit}[1]{\widehat{#1}}
\newcommand{\sign}[1]{\operatorname{sign}(#1)}
\newcommand{\vecangle}[2]{(#1,#2)}
\newcommand{\eqword}[1]{{\text{#1}}}

\newcommand{\gesLabel}[1]{{\texttt{#1}}}

%--------------------------------------------------
% common shortcuts in the text
%--------------------------------------------------
\usepackage{xspace}
\newcommand{\ie}{\textsl{i.e.}~}
\newcommand{\eg}{\textsl{e.g.}~}
\newcommand{\etal}{\textsl{et~al.}~}
\newcommand{\wrt}{\textsl{w.r.t.}~}
\newcommand{\NB}{\textsl{NB:}~}
\newcommand{\vs}{\textsl{vs.}~}
\newcommand{\cf}{\textsl{cf.}~}
\newcommand{\resp}{respectively\xspace}
\newcommand{\aka}{\textsl{a.k.a.}~}
\newcommand{\etc}{\textsl{etc.}}


%--------------------------------------------------
% Commands for keeping text (it's in the latex
%  but not displayed on pdf)
%--------------------------------------------------
\newcommand{\keep}[1]{}
\newcommand{\old}[1]{}

%--------------------------------------------------
% Math operators
%--------------------------------------------------
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mse}{mse}
\DeclareMathOperator*{\simloss}{sim}
\DeclareMathOperator*{\stopgrad}{sg}
\DeclareMathOperator*{\softmax}{softmax}
\newcommand{\norm}[1]{\lVert #1 \rVert}

%--------------------------------------------------
% References
%--------------------------------------------------
\usepackage{url}
\usepackage{hyperref}
% \usepackage{refcheck}
\newcommand{\fig}{Figure{}~}
\newcommand{\eqn}{Equation{}~}

%\captionsetup[figure]{singlelinecheck=off}
%\captionsetup[subfigure]{singlelinecheck=off}
%\captionsetup[table]{singlelinecheck=off}

%--------------------------------------------------
% Symboles
%--------------------------------------------------
% the generator state
\newcommand{\vrc}{\ensuremath{{\bm{o}}}}


==> sections/rebuttal.tex <==
\noindent We thank all the reviewers for their insightful suggestions and we will proofread our manuscript and fix all the typos.

\noindent\textcolor{VioletRed}{\textbf{[To Reviewer j8aN]}}
\textcolor{Blue}{\noindent\textbf{Q1: Dataset and code release.}}
\textcolor{Green}{\noindent\textbf{A1:}}
As stated in the supplementary, 
we will publicly release the full Streamer dataset upon acceptance. 
The dataset has been carefully anonymized and preprocessed for research use. 
In addition, we plan to release our training and inference code, as well as pre-trained models, to ensure that others can replicate and build upon our results with minimal effort.

\noindent\textcolor{Blue}{\textbf{Q2: Approach Extension.}}
\textcolor{Green}{\noindent\textbf{A2:} }\textbf{1)}
Thanks for the insightful question. 
Our Streamer dataset is, to our knowledge, the first to address the lack of instructional gesture data in live-streaming scenarios. 
Extending to multi-subject conversations is an meaningful, underexplored and more challenging direction, which we are actively exploring. An example from our ongoing two-person dataset construction is illustrated in Fig.1.
This requires additional processing, such as aligning speech segments with speaker identities using speech recognition and face identification. 
In terms of modeling, incorporating explicit interaction modules to handle multi-subject dynamics will also be necessary.

The proposed Hybrid Training strategy, Motion Style injection mechanism, and inference-time RAG strategy in HMDiT are generalizable and can be adapted to other audio-driven motion synthesis tasks. 
For instance, in Music-to-Dance Generation, the motion style input should capture not only person-specific features but also emphasize the influence of dance genre and music on the generated motion. In this context, keyframe selection should be guided more by musical rhythm rather than semantic cues.


\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{sec/img/issue.pdf}
\end{figure}


\noindent\textcolor{Blue}{\textbf{Q3: GPU requirements.}}
Our proposed HMDiT is not heavily dependent on computational resources. As noted in the main paper, we used a batch size of 512 with 40GB A100 GPU, and the model can also be trained on 24GB GPUs such as the RTX 3090 with less batch size. Moreover, both the encoder and decoder are lightweight, adding minimal overhead during training.

\noindent\textcolor{Blue}{\textbf{Q4: Explanation of FGD loss for ``w/o 3d kp loss''.}}
Similar to FID, FGD measures the distance between the feature distributions of GT and generated gestures. Introducing the 3d kp loss as a strong constraint reduces gesture diversity but improves the accuracy of generated gesture positions, benefiting downstream tasks like human video generation (see Fig.5 in paper).


\noindent\textcolor{VioletRed}{\textbf{[To Reviewer pej7]}}
\noindent\textcolor{Blue}{\textbf{Q1: Evaluation for RAG.}}
\noindent\textcolor{Green}{\textbf{A1:}} Thanks for your advice. We have evaluated RAG in the supplementary material; please refer to Section B.2 and Table 2. 


\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{sec/img/new_case.pdf}
\end{figure}


\noindent\textcolor{Blue}{\textbf{Q2: Diverse results.} }
\noindent\textcolor{Green}{\textbf{A2:}} Since our paper emphasizes the importance of instructional gestures, the results mainly feature numbers and directions. However, our dataset also contains global semantic and personalized gestures, as shown in Fig.2.

\noindent\textcolor{Blue}{\textbf{Q3: Dataset description.}}
\noindent\textcolor{Green}{\textbf{A3:}} Thanks for the advice. We will further improve the structure of the paper in future revisions, including the evaluation of RAG and the introduction of the dataset.

\noindent\textcolor{Blue}{\textbf{Q4: Figure 2 improvement.}}
\noindent\textcolor{Green}{\textbf{A4:}} We will further refine Figure 2 to present our method more clearly.

\noindent\textcolor{VioletRed}{\textbf{[To Reviewer mqvg]}}
\noindent\textcolor{Blue}{\textbf{Q1: Limited Dataset Diversity.}} 
\noindent\textcolor{Green}{\textbf{A1:}} 
We are building a gesture dataset across different cultures to further advance research in this field.
\noindent\textcolor{Blue}{\textbf{Q2: Baseline comparison with hybrid training.}} 
\noindent\textcolor{Green}{\textbf{A2:}} 
Our hybrid training strategy is not primarily designed to optimize BC. Instead, it aims to accelerate model convergence and enable controllable motion editing capabilities, which are crucial for downstream applications.
Moreover, our hybrid training scheme introduces no additional complexity or computational cost, except for a lightweight Keyframe Encoder.

\noindent\textcolor{Blue}{\textbf{Q3: Overlooked Sociocultural Factors.}}
\noindent\textcolor{Green}{\textbf{A3:} }
Thanks for your question. Our method generalizes well to other culturally specific hand gestures. For example, it can robustly generate the German hand gesture for the number three based on the corresponding key frame (see Fig.3).
%
As mentioned in Q1, we will 

\noindent\textcolor{Blue}{\textbf{Q4: Motion-style sequence selection.}}
\noindent\textcolor{Green}{\textbf{A4:}} The selected motion-style sequence is derived from another sequence of the same character, ensuring a clear content difference between the motion-style sequence and the input gesture. Moreover, we follow ~\cite{ji2022eamm} to conduct a ``temporal shuffle'' operation on the motion-style sequence for further disentanglement.

\noindent\textcolor{Blue}{\textbf{Q5: Details of automatic gesture annotation and SAR.}}
\textcolor{Green}{\textbf{A5:}}
For the SAR, we randomly select 450 generated results and corresponding GTs from test sets. Annotators are requested to label whether a semantic hand gesture is successfully triggered in each generated sequence: a score of 1 is given if triggered with the same hand as the GT, 0.5 if with the opposite hand, and 0 if not triggered. 
SAR is the ratio between the number of triggered sequences (scored 1 or 0.5) and the total number of generated sequences.

For automatic gesture annotation, we first select several reference DWPoses for each semantic gesture.
We locate gesture segments by using ASR to detect similar trigger words, extract and align DWPoses with the wrist root node, and determine inclusion in the semantic library based on similarity to reference poses.
